MICE: Minimal Interaction Cross-Encoders for efficient Re-ranking

In Information Retrieval (IR), cross-encoders deliver state-of-the-art ranking effectiveness but have a high inference cost, limiting their use to second-stage re-rankers. Prior work has addressed this bottleneck from two largely separate directions: accelerating cross-encoder inference through attention sparsification, or improving first-stage retrieval effectiveness to alleviate the need of a re-ranker, using more complex models, e.g. late-interactions. In this work, we bridge these two directions through an in-depth analysis of cross-encoder internal mechanisms. By identifying and removing superfluous interactions, we derive MICE (Minimal Interaction Cross-Encoders), a new cross-encoder architecture that retains effectiveness while reducing computational overhead. Extensive evaluations show MICE retains most of the performances of its cross-encoder counterparts in-domain and matches or even exceeds it in out-of-domain, while reducing FLOPs down to 2.5 times.

==> figures/Table2.tex <==
\begin{table*}[ht]
\centering
\caption{Re-ranking evaluation results over 1k docs/query from BM25 in nDCG@10 (over 5 seeds) for the experiments on MICE. Mask-X models are fine-tuned with \cref{mask_step:3} (see Section \ref{sec:masking}). ``MICE-$\ell$\texttt{X}+[\texttt{Y}/all]'' models indicates using only Y interaction layers (or all otherwise) starting from layer \texttt{X}. $ \uparrow $ and $ \downarrow $ marks a statistically significant difference between Mask or MICE models and their cross-encoder counterparts. \textbf{Bold} values marks the best averaged value per backbone, ``\textunderscore'' indicates second best. \hl{Gray} values indicate BM25 either matches or exceeds the baseline (corresp. average is reported in \textit{BM25-hard} column).}
%\vspace{-.3cm}
\resizebox{\textwidth}{!}{
\begin{tabular}{rlcccccccccccccccc|cc>{\columncolor{gray!20}}c}
\toprule
& &\multicolumn{3}{c}{\textbf{In-domain (ID)}} & \multicolumn{13}{c}{\textbf{BEIR (OOD)}} & \multicolumn{3}{c}{\textbf{Average}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-18}\cmidrule(lr){19-21}
\multicolumn{2}{l}{\textbf{Re-ranker}}  & MSM & DL19 & DL20 & Ar & CF & DB & FE & Fi & HPQ & NFC & NQ & Q & SD & SF & T-v2 & T-C & ID & OOD & BM25-hard \\
\midrule
\midrule
& BM25 & 23.0 & 51.2 & 47.7 & 30.0 & 16.5 & 31.8 & 65.1 & 23.6 & 63.3 & 32.2 & 30.6 & 78.9 & 14.0 & 67.9 & 45.4 & 59.5 & 42.5 & 43.0 & -\\
\multicolumn{2}{l}{ColBERTv2 \cite{santhanam2022colbertv2} \hf} & 45.0 & 74.6 & 73.4 & 33.8 & 17.0 & 44.3 & 73.0 & 34.2 & 66.2 & 33.4 & 53.9 & 86.3 & 14.1 & 63.8 & 34.2 & 66.7 & \textbf{64.3} & 47.8 & -\\
%aai-ColBERTv2-small  & \hf  & 42.4 & 74.0 & 70.3 & 33.8 & 26.5 & 45.7 & 85.6 & 38.2 & 76.8 & 35.4 & 57.1 & 87.6 & 17.9 & 72.4 & 28.5 & 80.8 & 62.2 & 52.8 \\
\midrule
\multirow{5}{*}{\rotatebox{90}{\textbf{MiniLM}}} 
& ColBERTv2  & 37.3 & 67.8 & 66.3 & 31.4 & 17.3 & 32.1 & 71.5 & 26.0 & 55.4 & 29.9 & 44.9 & 83.2 & 11.3 & 60.8 & 27.3 & 62.6 & 57.2 & 42.6 & 29.7 \\
\cmidrule{2-21}
 & \textbf{Baseline} & 44.7 & 73.8 & 72.9 & \cellcolor{gray!30} 14.8 & \cellcolor{gray!30} 15.7 & 46.0 & 73.4 & 34.0 & 72.4 & \cellcolor{gray!30} 27.1 & 56.6 & 80.4 & \cellcolor{gray!30} 12.5 & \cellcolor{gray!30} 55.3 & \cellcolor{gray!30} 29.9 & 63.4 & \textbf{63.8} & 44.7 & 25.9\\
 & \cref{mask_step:3}-$\ell$4  & 43.9 & 73.0 & 70.9 & 10.4 $\downarrow$ & 26.0 $\uparrow$ & 44.2 & 80.4 $\uparrow$ & 36.3 & 72.3 & 33.4 $\uparrow$ & 54.3 $\downarrow$ & 71.1 $\downarrow$ & 14.9 $\uparrow$ & 68.2 $\uparrow$ & 35.5 & 66.5 & \underline{62.6} & 47.2 & \underline{31.4} \\
 & MICE-$\ell$4+all & 43.1 $\downarrow$ & 73.4 & 70.1 & 39.0 $\uparrow$ & 25.1 $\uparrow$ & 44.4 & 79.1 $\uparrow$ & 35.6 & 72.0 & 34.5 $\uparrow$ & 52.2 $\downarrow$ & 81.4 $\uparrow$ & 14.8 $\uparrow$ & 70.5 $\uparrow$ & 39.4 $\uparrow$ & 69.2 & 62.2 & \textbf{50.5} & \textbf{37.2} \\
 & MICE-$\ell$4+3 & 42.1 $\downarrow$ & 72.6 & 69.3 & 41.0 $\uparrow$ & 24.4 $\uparrow$ & 43.7 & 79.8 $\uparrow$ & 34.7 & 71.3 $\downarrow$ & 34.3 $\uparrow$ & 51.4 $\downarrow$ & 81.4 $\uparrow$ & 14.9 $\uparrow$ & 69.2 $\uparrow$ & 39.5 $\uparrow$ & 69.4 & 61.3 & \underline{50.4} & \textbf{37.2} \\
 %& MICE-$\ell$6+4 & 42.6 $\downarrow$ & 69.2 & 69.8 & 36.2 $\uparrow$ & 25.6 $\uparrow$ & 41.9 $\downarrow$ & 78.1 $\uparrow$ & 35.4 & 69.3 $\downarrow$ & 34.1 $\uparrow$ & 51.7 $\downarrow$ & 81.2 $\uparrow$ & 14.4 $\uparrow$ & 69.9 $\uparrow$ & 38.4 & 68.7 & 60.6 & 49.6 \\
 
\midrule
\midrule
\multirow{4}{*}{\rotatebox{90}{\textbf{Ettin-32M}}} 
 & \textbf{Baseline} & 42.8 & 70.5 & 69.3 & \cellcolor{gray!30} 12.0 & 23.4 & 41.1 & 82.3 & 36.4 & 69.5 & 33.7 & 52.1 & \cellcolor{gray!30} 79.0 & \cellcolor{gray!30} 14.5 & 68.8 & \cellcolor{gray!30} 41.2 & 72.0 & \textbf{60.9} & \textbf{48.2} & 36.7\\
 & \cref{mask_step:3}-$\ell$6 & 41.9 & 69.4 & 68.6 & 9.2 $\downarrow$ & 22.9 & 37.8 & 78.3 $\downarrow$ & 34.4 & 65.0 $\downarrow$ & 32.8 & 49.8 $\downarrow$ & 37.8 $\downarrow$ & 12.4 $\downarrow$ & 66.8 & 40.8 & 68.7 & 59.9 & 42.8 & 25.1  \\
 & MICE-$\ell$6+all & 42.4 & 70.3 & 69.5 & 14.8 $\uparrow$ & 21.6 $\downarrow$ & 39.7 & 71.6 $\downarrow$ & 26.2 $\downarrow$ & 68.0 $\downarrow$ & 32.9 & 49.1 $\downarrow$ & 82.4 $\uparrow$ & 11.9 $\downarrow$ & 68.4 & 41.9 & 72.9 & \underline{60.7} & 46.3 & \underline{37.8}  \\
 & MICE-$\ell$6+3& 41.9 $\downarrow$ & 69.3 & 68.4 & 18.8 $\uparrow$ & 21.6 $\downarrow$ & 38.9 & 71.5 $\downarrow$ & 27.3 $\downarrow$ & 67.3 $\downarrow$ & 32.8 & 48.5 $\downarrow$ & 82.0 $\uparrow$ & 11.9 $\downarrow$ & 68.9 & 41.9 & 71.5 & 59.8 & \underline{46.4} & \textbf{38.7} \\

\midrule
\multirow{4}{*}{\rotatebox{90}{\textbf{Ettin-17M}}} 
 & \textbf{Baseline} & 38.6 & 64.9 & 63.6 & \cellcolor{gray!30} 12.9 & 21.0 & 33.6 & 77.5 & 31.0 & \cellcolor{gray!30} 60.5 & \cellcolor{gray!30} 31.5 & 45.7 & \cellcolor{gray!30} 76.7 & \cellcolor{gray!30} 12.2 & \cellcolor{gray!30} 66.1 & \cellcolor{gray!30} 36.4 & 66.7 & \textbf{55.7} & \textbf{44.0} & 42.3\\
 & \cref{mask_step:3}-$\ell$3   & 37.8 & 66.1 & 62.4 & 14.0 & 22.9 $\uparrow$ & 33.1 & 73.8 $\downarrow$ & 29.3 & 62.1 $\uparrow$ & 30.6 & 44.3 & 71.4 $\downarrow$ & 11.9 & 62.9 & 41.2 & 64.9 & \underline{55.4} & 43.3 & 42.0 \\
 & MICE-$\ell$3+all & 37.7 & 66.1 & 62.2 & 20.1 $\uparrow$ & 19.1 $\downarrow$ & 33.3 & 68.0 $\downarrow$ & 24.4 $\downarrow$ & 62.0 $\uparrow$ & 29.9 & 42.8 $\downarrow$ & 81.3 $\uparrow$ & 9.6 $\downarrow$ & 67.0 & 40.2 & 66.6 & 55.3 & 43.4 & \underline{44.3} \\
 & MICE-$\ell$3+3 & 38.0 & 65.7 & 62.4 & 20.2 $\uparrow$ & 19.1 $\downarrow$ & 33.9 & 67.5 $\downarrow$ & 24.5 $\downarrow$ & 63.1 $\uparrow$ & 29.9 & 43.1 $\downarrow$ & 80.8 $\uparrow$ & 9.2 $\downarrow$ & 67.3 & 44.2 & 67.3 & \underline{55.4} & \underline{43.9} & \textbf{44.9} \\
\bottomrule
\end{tabular}
}
\label{tab:MICE-evals}
%\vspace{-.3cm}
\end{table*}

% \begin{table*}[ht]
% \centering
% \caption{Re-ranking evaluation results over 1k docs/query from BM25 in nDCG@10 (over 5 seeds) for the experiments on MICE. Mask-X models are fine-tuned with \cref{mask_step:3} (see Section \ref{sec:masking}). ``MICE-$\ell$\texttt{X}+[\texttt{Y}/all]'' models indicates interaction layers start with layer \texttt{X}, and end at layer \texttt{Y} (or all otherwise). $ \uparrow $ and $ \downarrow $ marks a statistically significant difference between Mask or MICE models and their cross-encoder counterparts. \textbf{Bold} values marks the best averaged value per backbone, ``\textunderscore'' indicates second best.}
% \vspace{-.3cm}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{rlcccccccccccccccc|cc}
% \toprule
% & &\multicolumn{3}{c}{\textbf{In-domain}} & \multicolumn{13}{c}{\textbf{BEIR (OOD)}} & \multicolumn{4}{c}{\textbf{Average}} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-18}\cmidrule(lr){19-220}
% \multicolumn{2}{l}{\textbf{Re-ranker}}  & MSM & DL19 & DL20 & Ar & CF & DB & FE & Fi & HPQ & NFC & NQ & Q & SD & SF & T-v2 & T-C & ID & OOD \\
% \midrule
% \midrule
% & BM25 & 23.0 & 51.2 & 47.7 & 30.0 & 16.5 & 31.8 & 65.1 & 23.6 & 63.3 & 32.2 & 30.6 & 78.9 & 14.0 & 67.9 & 45.4 & 59.5 & 42.5 & 43.0 \\
% \multicolumn{2}{l}{ColBERTv2 \cite{santhanam2022colbertv2} \hf} & 45.0 & 74.6 & 73.4 & 33.8 & 17.0 & 44.3 & 73.0 & 34.2 & 66.2 & 33.4 & 53.9 & 86.3 & 14.1 & 63.8 & 34.2 & 66.7 & \textbf{64.3} & 47.8 \\
% %aai-ColBERTv2-small  & \hf  & 42.4 & 74.0 & 70.3 & 33.8 & 26.5 & 45.7 & 85.6 & 38.2 & 76.8 & 35.4 & 57.1 & 87.6 & 17.9 & 72.4 & 28.5 & 80.8 & 62.2 & 52.8 \\
% \midrule
% \multirow{5}{*}{\rotatebox{90}{\textbf{MiniLM}}} 
% & ColBERTv2  & 37.3 & 67.8 & 66.3 & 31.4 & 17.3 & 32.1 & 71.5 & 26.0 & 55.4 & 29.9 & 44.9 & 83.2 & 11.3 & 60.8 & 27.3 & 62.6 & 57.2 & 42.6 \\
% \cmidrule{2-20}
%  & \textbf{Baseline} & 44.7 & 73.8 & 72.9 & \cellcolor{gray!30} 14.8 & \cellcolor{gray!30} 15.7 & 46.0 & 73.4 & 34.0 & 72.4 & \cellcolor{gray!30} 27.1 & 56.6 & 80.4 & \cellcolor{gray!30} 12.5 & \cellcolor{gray!30} 55.3 & \cellcolor{gray!30} 29.9 & 63.4 & \textbf{63.8} & 44.7 \\
%  & \cref{mask_step:3}-$\ell$4   & 43.9 & 73.0 & 70.9 & 10.4 $\downarrow$ & 26.0 $\uparrow$ & 44.2 & 80.4 $\uparrow$ & 36.3 & 72.3 & 33.4 $\uparrow$ & 54.3 $\downarrow$ & 71.1 $\downarrow$ & 14.9 $\uparrow$ & 68.2 $\uparrow$ & 35.5 & 66.5 & \underline{62.6} & 47.2 \\
%  & MICE-$\ell$4+all & 43.1 $\downarrow$ & 73.4 & 70.1 & 39.0 $\uparrow$ & 25.1 $\uparrow$ & 44.4 & 79.1 $\uparrow$ & 35.6 & 72.0 & 34.5 $\uparrow$ & 52.2 $\downarrow$ & 81.4 $\uparrow$ & 14.8 $\uparrow$ & 70.5 $\uparrow$ & 39.4 $\uparrow$ & 69.2 & 62.2 & \textbf{50.5} \\
%  & MICE-$\ell$4+3 & 42.1 $\downarrow$ & 72.6 & 69.3 & 41.0 $\uparrow$ & 24.4 $\uparrow$ & 43.7 & 79.8 $\uparrow$ & 34.7 & 71.3 $\downarrow$ & 34.3 $\uparrow$ & 51.4 $\downarrow$ & 81.4 $\uparrow$ & 14.9 $\uparrow$ & 69.2 $\uparrow$ & 39.5 $\uparrow$ & 69.4 & 61.3 & \underline{50.4} \\
%  %& MICE-$\ell$6+4 & 42.6 $\downarrow$ & 69.2 & 69.8 & 36.2 $\uparrow$ & 25.6 $\uparrow$ & 41.9 $\downarrow$ & 78.1 $\uparrow$ & 35.4 & 69.3 $\downarrow$ & 34.1 $\uparrow$ & 51.7 $\downarrow$ & 81.2 $\uparrow$ & 14.4 $\uparrow$ & 69.9 $\uparrow$ & 38.4 & 68.7 & 60.6 & 49.6 \\
 
% \midrule
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textbf{Ettin-32M}}} 
%  & \textbf{Baseline} & 42.8 & 70.5 & 69.3 & \cellcolor{gray!30} 12.0 & 23.4 & 41.1 & 82.3 & 36.4 & 69.5 & 33.7 & 52.1 & \cellcolor{gray!30} 79.0 & \cellcolor{gray!30} 14.5 & 68.8 & \cellcolor{gray!30} 41.2 & 72.0 & \textbf{60.9} & \textbf{48.2} \\
%  & \cref{mask_step:3}-$\ell$6 & 41.9 & 69.4 & 68.6 & 9.2 $\downarrow$ & 22.9 & 37.8 & 78.3 $\downarrow$ & 34.4 & 65.0 $\downarrow$ & 32.8 & 49.8 $\downarrow$ & 37.8 $\downarrow$ & 12.4 $\downarrow$ & 66.8 & 40.8 & 68.7 & 59.9 & 42.8 \\
%  & MICE-$\ell$6+all & 42.4 & 70.3 & 69.5 & 14.8 $\uparrow$ & 21.6 $\downarrow$ & 39.7 & 71.6 $\downarrow$ & 26.2 $\downarrow$ & 68.0 $\downarrow$ & 32.9 & 49.1 $\downarrow$ & 82.4 $\uparrow$ & 11.9 $\downarrow$ & 68.4 & 41.9 & 72.9 & \underline{60.7} & 46.3 \\
%  & MICE-$\ell$6+3& 41.9 $\downarrow$ & 69.3 & 68.4 & 18.8 $\uparrow$ & 21.6 $\downarrow$ & 38.9 & 71.5 $\downarrow$ & 27.3 $\downarrow$ & 67.3 $\downarrow$ & 32.8 & 48.5 $\downarrow$ & 82.0 $\uparrow$ & 11.9 $\downarrow$ & 68.9 & 41.9 & 71.5 & 59.8 & \underline{46.4} \\

% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textbf{Ettin-17M}}} 
%  & \textbf{Baseline} & 38.6 & 64.9 & 63.6 & \cellcolor{gray!30} 12.9 & 21.0 & 33.6 & 77.5 & 31.0 & \cellcolor{gray!30} 60.5 & \cellcolor{gray!30} 31.5 & 45.7 & \cellcolor{gray!30} 76.7 & \cellcolor{gray!30} 12.2 & \cellcolor{gray!30} 66.1 & \cellcolor{gray!30} 36.4 & 66.7 & \textbf{55.7} & \textbf{44.0} \\
%  & \cref{mask_step:3}-$\ell$3   & 37.8 & 66.1 & 62.4 & 14.0 & 22.9 $\uparrow$ & 33.1 & 73.8 $\downarrow$ & 29.3 & 62.1 $\uparrow$ & 30.6 & 44.3 & 71.4 $\downarrow$ & 11.9 & 62.9 & 41.2 & 64.9 & \underline{55.4} & 43.3 \\
%  & MICE-$\ell$3+all & 37.7 & 66.1 & 62.2 & 20.1 $\uparrow$ & 19.1 $\downarrow$ & 33.3 & 68.0 $\downarrow$ & 24.4 $\downarrow$ & 62.0 $\uparrow$ & 29.9 & 42.8 $\downarrow$ & 81.3 $\uparrow$ & 9.6 $\downarrow$ & 67.0 & 40.2 & 66.6 & 55.3 & 43.4 \\
%  & MICE-$\ell$3+3 & 38.0 & 65.7 & 62.4 & 20.2 $\uparrow$ & 19.1 $\downarrow$ & 33.9 & 67.5 $\downarrow$ & 24.5 $\downarrow$ & 63.1 $\uparrow$ & 29.9 & 43.1 $\downarrow$ & 80.8 $\uparrow$ & 9.2 $\downarrow$ & 67.3 & 44.2 & 67.3 & \underline{55.4} & \underline{43.9} \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:MICE-evals}
% \vspace{-.3cm}
% \end{table*}

%%% Discarded results 
 % & MICE-$\ell$4+all & 40.7 $\downarrow$ & 68.8 & 68.1 & 9.1 $\downarrow$ & 19.0 $\downarrow$ & 37.5 $\downarrow$ & 69.5 $\downarrow$ & 25.6 $\downarrow$ & 63.9 $\downarrow$ & 31.3 & 45.5 $\downarrow$ & 80.3 & 10.1 $\downarrow$ & 65.8 & 39.2 & 67.1 & 59.2 & 43.4 \\
 % & \cref{mask_step:3}-$\ell$4 & 42.2 & 69.5 & 69.4 & 13.0 & 23.0 & 38.5 & 79.0 $\downarrow$ & 34.9 & 66.1 $\downarrow$ & 33.0 & 50.4 $\downarrow$ & 39.6 $\downarrow$ & 12.8 $\downarrow$ & 67.8 & 41.4 & 69.5 & 60.3 & 43.8 \\
 % & MICE-$\ell$4+3& 39.4 $\downarrow$ & 68.2 & 65.5 & 13.5 $\uparrow$ & 14.9 $\downarrow$ & 34.9 $\downarrow$ & 65.4 $\downarrow$ & 19.9 $\downarrow$ & 63.6 $\downarrow$ & 29.3 & 43.4 $\downarrow$ & 80.4 $\uparrow$ & 7.2 $\downarrow$ & 61.4 $\downarrow$ & 44.5 & 64.7 & 57.7 & 41.8 \\

==> figures/Table3.tex <==
\begin{table}[!h]
\centering
\caption{Re-ranking evaluation results over 1k docs/query from BM25 in nDCG@10 (over 5 seeds) for the experiments towards scaling MICE to bigger models.  $ \uparrow $ and $ \downarrow $ marks a statistically significant difference between a MICE model and its cross-encoder counterpart.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{rccccc}
\toprule
\textbf{Model} & \textbf{F} & MSM & DL19 & DL20 & Avg\\
\midrule
BM25 &  & 23.0 & 51.2 & 47.7 & 42.5 \\
\midrule
MiniLM &  & 44.7 & 73.8 & 72.9 & 63.8 \\
% MICE(MiniLM) & $\ell$6+4  & 42.6 $\downarrow$ & 69.2 & 69.8 & 60.6 \\
MICE(MiniLM) & $\ell$4+3  & 42.1 $\downarrow$ & 72.6 & 69.3 & 61.3 \\
\midrule
Ettin-17M & & 38.6 & 64.9 & 63.6 & 55.7 \\
%MICE(Ettin-17M) & $\ell$3+2 & 36.6 $\downarrow$ & 65.4 & 60.6 & 54.2 \\
MICE(Ettin-17M) & $\ell$3+3 & 38.0 & 65.7 & 62.4 & 55.4 \\
\midrule
Ettin-32M &  & 42.8 & 70.5 & 69.3 & 60.9 \\
% MICE(Ettin-32M) & $\ell$4+3 & 39.4 $\downarrow$ & 68.2 & 65.5 & 57.7 \\
%MICE(Ettin-32M) & $\ell$6+2 & 41.4 $\downarrow$ & 69.5 & 68.7 & 59.9 \\
MICE(Ettin-32M) & $\ell$6+3 & 41.9 $\downarrow$ & 69.3 & 68.4 & 59.8 \\
\midrule
Ettin-68M &  & 45.7 & 74.1 & 73.8 & 64.5 \\
MICE(Ettin-68M) & $\ell$7+3 & 42.6 $\downarrow$ & 70.2 & 69.3 & 60.7 \\
MICE(Ettin-68M) & $\ell$10+3 & 43.6 $\downarrow$ & 73.0 & 70.7 & 62.4 \\
\midrule
Ettin-150M &  & 46.4 & 75.1 & 74.1 & 65.2 \\
MICE(Ettin-150M) & $\ell$8+3 & 44.6 $\downarrow$ & 73.3 & 71.8 & 63.2 \\
MICE(Ettin-150M) & $\ell$11+3 & 45.0 $\downarrow$ & 74.4 & 71.9 & 63.8 \\
\bottomrule
\end{tabular}
}
\label{tab:MICE-scaling}
\end{table}
